Investigation of inverse design of multilayer thin-films with conditional invertible Neural Networks

The task of designing optical multilayer thin-films regarding a given target is currently solved using gradient-based optimization in conjunction with methods that can introduce additional thin-film layers. Recently, Deep Learning and Reinforcement Learning have been been introduced to the task of designing thin-films with great success, however a trained network is usually only able to become proficient for a single target and must be retrained if the optical targets are varied. In this work, we apply conditional Invertible Neural Networks (cINN) to inversely designing multilayer thin-films given an optical target. Since the cINN learns the energy landscape of all thin-film configurations within the training dataset, we show that cINNs can generate a stochastic ensemble of proposals for thin-film configurations that that are reasonably close to the desired target depending only on random variables. By refining the proposed configurations further by a local optimization, we show that the generated thin-films reach the target with significantly greater precision than comparable state-of-the art approaches. Furthermore, we tested the generative capabilities on samples which are outside the training data distribution and found that the cINN was able to predict thin-films for out-of-distribution targets, too. The results suggest that in order to improve the generative design of thin-films, it is instructive to use established and new machine learning methods in conjunction in order to obtain the most favorable results.

==> 2_state_of_the_art.tex <==
Often, heuristic approaches are required to tackle a new problem as no existing algorithm solves the problem efficiently. With the rise of machine learning in the recent years reinforcement learning has been the go to method to teach a neural network to develop a design strategy and implicitly optimize the design through q-value estimation. As reinforcement learning is based on strategy optimization, it lacks a fundamental understanding of the physical properties and relies on a physical model to validate new designs. This approach is therefore not feasible for possibly expensive simulations. The necessity of a fast-to-evaluate physical model has been removed by surrogate modelling as demonstrated by Peurifoy et. al. \cite{surrogate_model_inverse_design}. Their neural network surrogate model is capable of optimizing the optical response of a nanoparticle ensemble while outperforming classical algorithms but lack inherent mechanisms to deal with ambiguous designs. Flow based generative networks \cite{kingma2018glow, flow_gan, i-rev_net, abdal2020styleflow} are mostly used in image synthesis and integrate other techniques, too, such as adversarial training. An interesting advantage over adversarial training is that invertible networks based on normalizing flows can learn the inverse pass through the network implicitly by training only on the well understood forward process. The principle applicability of INNs to physical problems was demonstrated by Ardizzonne et. al. \cite{ardizzone2019analyzing}. They applied an INN to estimate properties from interstellar molecular clouds.


